emucxl: an emulation framework for CXL-based disaggregated memory applications

The emergence of CXL (Compute Express Link) promises to transform the status of interconnects between host and devices and in turn impact the design of all software layers. With its low overhead, low latency, and memory coherency capabilities, CXL has the potential to improve the performance of existing devices while making viable new operational use cases (e.g., disaggregated memory pools, cache coherent memory across devices etc.). The focus of this work is design of applications and middleware with use of CXL for supporting disaggregated memory. A vital building block for solutions in this space is the availability of a standard CXL hardware and software platform. Currently, CXL devices are not commercially available, and researchers often rely on custom-built hardware or emulation techniques and/or use customized software interfaces and abstractions. These techniques do not provide a standard usage model and abstraction layer for CXL usage, and developers and researchers have to reinvent the CXL setup to design and test their solutions, our work aims to provide a standardized view of the CXL emulation platform and the software interfaces and abstractions for disaggregated memory. This standardization is designed and implemented as a user space library, emucxl and is available as a virtual appliance. The library provides a user space API and is coupled with a NUMA-based CXL emulation backend. Further, we demonstrate usage of the standardized API for different use cases relying on disaggregated memory and show that generalized functionality can be built using the open source emucxl library.

==> sections/scope.tex <==


\teal{The scope of this work mainly revolves around standardizing CXL emulation 
framework and building open source software interfaces and abstractions for 
disaggregated memory. Why this is implement and relevant for the computing world?
CXL being the new technology and no real hardware availability indirectly pushes the
researchers and developers to build or reinvent custom-built hardware or software
solutions. Our work offers researchers and developers a viable alternative in the form of standardized emulation framework and software interfaces called \emucxl, so that researchers
and developers can efficiently design, prototype, and validate their CXL-based solutions 
without the need of building or reinventing custom solutions consumes significant time,
effort, and resources, which could be better utilized for actual research and innovation.}

\teal{Until commercial CXL hardware becomes available and is supported by
operating systems with dedicated software runtimes, or alternatively, until
emulation using solutions 
% like QEMU
is utilized, our work \Emucxl presents
a promising candidate for advancing research in the field of disaggregated
memory using CXL. By providing a standardized framework and software 
interfaces, \Emucxl can effectively support and enhance research efforts
in exploring the capabilities and potential of CXL-enabled systems. 
Its standardized approach will enable researchers to develop and test applications and
solutions that leverage disaggregated memory at a faster pace.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Requirements %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Requirements}
\label{subsection:requirements}
\raja{Does this subsection required? We can merge this scope of work
section itself.}
\teal{
We are standardizing Pond's cxl emulation
technique to a view of the CXL emulation platform and
abstractions for disaggregated memory. Further, this standardization effort
will greatly benefit developers and researchers, as they won't have to start 
from scratch to design and test their solutions for CXL disaggregated memory
usage.
\begin{itemize}
    \item 2-socket physical server as the underlying hardware
    \item VM creation using QEMU (hypervisor)
    \item VM emulate a single-socket system on a two-socket physical server
    by disabling all cores in one socket, while keeping its memory accessible
    from the other socket.
\end{itemize}
}
\raja{Is a figure showing modified(i.e for multiple vm) pond design required here?}
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{images/pond.png}
    \caption{Standardized CXL emulation}
    \label{fig:pond}
\end{figure}
\raja{Figure ~\ref{fig:pond}. Looks good?}
\teal{The standardized API is designed and implemented as a user space
library, \emucxl. This library offers a comprehensive user space API 
and is complemented by a NUMA-based CXL emulation backend. The 
NUMA-based backend leverages NUMA-aware memory allocation semantics 
and is implemented as a Linux kernel module. To successfully deploy
the \Emucxl library and its accompanying backend, it is recommended 
to use an Ubuntu version, preferably 22.04, with a kernel version 
equal to or greater than 5.15. This software configuration ensures
compatibility for the successful execution of the \Emucxl functionality.}


% \end{document}
